Accelerator and Beam Physics: Grand Challenges and Research Opportunities

Accelerator and beam physics (ABP) is the science of the motion, generation, acceleration, manipulation, prediction, observation and use of charged particle beams. It focuses on fundamental long-term accelerator and beam physics research and development. Accelerator and beam physics research has resulted in important advances in accelerator science, yet support for this research is declining. NSF has terminated its program in accelerator Science and funding by DOE through GARD and Accelerator Stewardship has been steady or declining. The declining support for accelerator research will slow advances and threaten student training and work-force development in accelerator science. We propose a robust and scientifically challenging program in accelerator and beam physics, which will position the field of US High Energy Physics to be productive and competitive for decades to come.

==> workshopsymbols.tex <==
%%%%   Standard symbols for use in Snowmass Working Group Proceedings%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  basic formatting macros:%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%   text mode macros

\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\ibid{{\it ibid}.}

\def\Acknowledgements{\bigskip  \bigskip \begin{center} \begin{large}
             \bf ACKNOWLEDGEMENTS \end{large}\end{center}}


%  equation display macros

\def\beq{\begin{equation}}
\def\eeq#1{\label{#1}\end{equation}}
\def\eeqn{\end{equation}}

%%  multiple-line equations  (use \CR as the carriage return):

\newenvironment{Eqnarray}%
   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
\def\beqa{\begin{Eqnarray}}
\def\eeqa#1{\label{#1}\end{Eqnarray}}
\def\eeqan{\end{Eqnarray}}
\def\CR{\nonumber \\ }

%%  reference to an equation number:

\def\leqn#1{(\ref{#1})}

%%  sizing and bars

\def\st{\scriptstyle}
\def\sst{\scriptscriptstyle}

\def\overbar#1{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar

\def\subscr#1{{\mbox{\scriptsize #1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  expectation values: 

\def\VEV#1{\left\langle{ #1} \right\rangle}
\def\bra#1{\left\langle{ #1} \right|}
\def\ket#1{\left| {#1} \right\rangle}
\def\vev#1{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% relation symbols

\def\lsim{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\gsim{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}

\def\Im{{\rm Im}}
\def\Re{{\rm Re}}
\def\tr{{ \rm tr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  caligraphic letters (for matrix elements, luminosity, etc.)

\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}
\def\H{{\cal H}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  matrix operations and fractions:

\def\One{{\bf 1}}
\def\hc{{\mbox{\rm h.c.}}}
\def\tr{{\mbox{\rm tr}}}
\def\half{\frac{1}{2}}
\def\thalf{\frac{3}{2}}
\def\third{\frac{1}{3}}
\def\tthird{\frac{2}{3}}

\def\del{\partial}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}
\def\pslash{\not{\hbox{\kern-2pt $p$}}}
\def\ETmiss{\not{\hbox{\kern-4pt $E$}}_T}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  high-energy physics terminology:

\def\Pl{{\mbox{\scriptsize Pl}}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\GUT{{\mbox{\scriptsize GUT}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\gw{\Gamma_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_H}
\def\gh{\Gamma_H}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\MSB{{\bar{M \kern -2pt S}}}
\def\msb{{\bar{\scriptsize M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\drb{{\bar{\scriptsize D \kern -1pt R}}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}
\def\Kzero{K^0}
\def\Kzerobar{{\bar K}^0}
\def\Dzero{D^0}
\def\Dzerobar{{\bar D}^0}
\def\Bzero{B^0}
\def\Bzerobar{{\bar B}^0}


%%%%%%%%%%%%   units for math mode  %%%%%%%%%%%%%%%%%%%%%%%%%

\def\ifb{{\rm fb}^{-1}}
\def\eV{{\rm eV}}
\def\keV{{\rm keV}}
\def\MeV{{\rm MeV}}
\def\GeV{{\rm GeV}}
\def\TeV{{\rm TeV}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  supersymmetry:

\def\ch#1{\widetilde\chi^+_{#1}}
\def\chm#1{\widetilde\chi^-_{#1}}
\def\neu#1{\widetilde\chi^0_{#1}}
\def\s#1{\widetilde{#1}}



%%%%%%%%%%  common journal names   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\aj{{Astronomical Journal}}%
\newcommand\araa{{Annual Review of Astron and Astrophys}}%
 \newcommand\apj{{Astrophysical Journal}}%
\newcommand\apjl{{Astrophysical Journal, Letters}}%
\newcommand\apjs{{ApJS}}%
% Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}%
% Applied Optics
\newcommand\apss{{Ap\&SS}}%
% Astrophysics and Space Science
\newcommand\aap{{Astronomy and Astrophysics}}%
\newcommand\aapr{{A\&A~Rev.}}%
% Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}%
% Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}%
% Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}%
% Bulletin of the AAS
\newcommand\jrasc{{JRASC}}%
% Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}%
% Memoirs of the RAS
\newcommand\mnras{{Monthly Notices of the Royal Astronomical Society}}%
\newcommand\pra{{Phys.~Rev.~A}}%
% Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}%
% Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}%
% Physical Review C
\newcommand\prd{{Physics~Review~D}}%
% Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}%
% Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}%
% Physical Review Letters
\newcommand\pasp{{Publications of the ASP}}%
\newcommand\pasj{{PASJ}}%
% Publications of the ASJ
\newcommand\qjras{{QJRAS}}%
% Quarterly Journal of the RAS
\newcommand\jcap{{JCAP}}%
\newcommand\skytel{{S\&T}}%
% Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}%
% Solar Physics
\newcommand\sovast{{Soviet~Ast.}}%
% Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}%
% Space Science Reviews
\newcommand\zap{{ZAp}}%
% Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}%
\newcommand\iaucirc{{IAU~Circ.}}%
% IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}}%
% Astrophysics Letters
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}%
% Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}%
% Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}%
% Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}%
% Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}}%
% Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}%
% Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}%
% Journal of Geophysics Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}%
% Journal of Quantitative Spectroscopy and Radiative Transfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}%
% Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}%
% Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}%
% Physics Reports
\newcommand\physscr{{Phys.~Scr}}%
% Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}%
% Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
